An Interpretable Two-Stage Feature Decomposition Method for Deep Learning-based SAR ATR

Synthetic aperture radar automatic target recognition (SAR ATR) has seen significant performance improvements with deep learning. However, the black-box nature of deep SAR ATR introduces low confidence and high risks in decision-critical SAR applications, hindering practical deployment. To address this issue, deep SAR ATR should provide an interpretable reasoning basis $r_b$ and logic $\lambda_w$, forming the reasoning logic $\sum_{i} {{r_b^i} \times {\lambda_w^i}} =pred$ behind the decisions. Therefore, this paper proposes a physics-based two-stage feature decomposition method for interpretable deep SAR ATR, which transforms uninterpretable deep features into attribute scattering center components (ASCC) with clear physical meanings. First, ASCCs are obtained through a clustering algorithm. To extract independent physical components from deep features, we propose a two-stage decomposition method. In the first stage, a feature decoupling and discrimination module separates deep features into approximate ASCCs with global discriminability. In the second stage, a multilayer orthogonal non-negative matrix tri-factorization (MLO-NMTF) further decomposes the ASCCs into independent components with distinct physical meanings. The MLO-NMTF elegantly aligns with the clustering algorithms to obtain ASCCs. Finally, this method ensures both an interpretable reasoning process and accurate recognition results. Extensive experiments on four benchmark datasets confirm its effectiveness, showcasing the method's interpretability, robust recognition performance, and strong generalization capability.

==> material/material_ASC.tex <==

\begin{algorithm}
    \caption{K-means Clustering Algorithm}
    \begin{algorithmic}[1]
        \REQUIRE ~~\\ %算法的输入参数：Input
        The set of ASC parameters of target, $P = \{p_1, p_2, \dots, p_n\}$;\\
        The number of clusters, $K$.\\
        
        \ENSURE ~~\\The final cluster centers and cluster labels for ASC parameters $P$.
        
        \STATE Randomly choose $K$ initial cluster centers $\{c_1, c_2, \dots, c_k\}$
        \REPEAT
        \STATE For each ASC $p_i$, compute its distance to each  center:
        \[
        \text{d}(p_i, c_j) = \| p_i - c_j \|^2,  \forall i \in \{1, 2, \dots, n\},  \forall j \in \{1, 2, \dots, K\}
        \]
        \STATE Assign $p_i$ to the nearest cluster center:
        \[
        c(p_i) = \arg \min_j \| x_i - c_j \|^2,  \forall i \in \{1, 2, \dots, n\}
        \]
        \STATE Update each cluster center:
        \[
        c_j = \frac{1}{|C_j|} \sum_{p_i \in C_j} p_i, \forall j \in \{1, 2, \dots, K\}
        \]
        \UNTIL Cluster centers do not change or the maximum number of iterations is reached
        
    \end{algorithmic}
\end{algorithm}



% \begin{figure}[tb]
% \centering
% \includegraphics[width=0.3\textwidth]{fig_asc/ASC_extraction.pdf} 
% \caption{Flowchart of SAR ASC Component Extraction.}
% \label{asc_extraction}
% \end{figure}

==> material/method_NMF.tex <==
\subsection{Multi-layer Orthogonal NMTF} \label{methodsec2}



Now the data matrix $X\in \mathbb{R}^{m \times n}$ is non-negative.
We use non-negative matrix tri-factorization \cite{choi2008algorithms} to decompose it into three matrices,
\begin{equation}\label{equ: X=U1W1V1}
    X\approx U_{1}W_{1}V_{1}^{\top}
\end{equation}
where $U_{1} \in \mathbb{R}^{m \times r}$ and $V_{1} \in \mathbb{R}^{n \times r}$ are orthogonal matrices satisfing $U_{1}^{\top}U_{1} = I$ and $V_{1}^{\top}V_{1}=I$, $r$ is the target rank. 
This ensures that the matrix $W_{1}\in \mathbb{R}^{r \times r}$ is a low-rank approximation of $X$ resulting from co-clustering \cite{ding2005equivalence}.
We consider the squared Euclidean distance as a discrepancy measure between the data $X$ and the model $U_{1}W_{1}V_{1}^{\top}$, non-negative matrix tri-factorization involves the following optimization,
\begin{equation}\label{equ: J = X-U1W1V1}
    \begin{aligned}
    & \underset{U_{1}\geq 0,W_{1}\geq 0,V_{1}\geq 0}{\text{minimize}}
    & & \mathcal{J}(U_{1},W_{1},V_{1}) = \frac{1}{2}\|X-U_{1}W_{1}V_{1}^{\top}\|_{F}^{2}  \\
    & \text{subject to}
    & & U_{1}^{\top}U_{1} = I \text{ and } V_{1}^{\top}V_{1}=I.
\end{aligned}
\end{equation}

Yoo and Choi \cite{yoo2010orthogonal} gave a multiplicative algorithm for non-negative matrix tri-factorization.
Suppose that the gradient of an optimization function $\mathcal{J}$ has a decomposition that is of the form,
\begin{equation}\label{equ: J = J+ - J-}
    \nabla \mathcal{J} = [\nabla \mathcal{J}]^{+}-[\nabla \mathcal{J}]^{-},
\end{equation}
where $[\nabla \mathcal{J}]^{+}>0$ and $[\nabla \mathcal{J}]^{-}>0$. 
Then multiplicative update for parameters $\Theta$ has the form
\begin{equation}\label{equ: Theta <- Theta}
    \Theta \leftarrow \Theta \odot \left(\frac{[\nabla \mathcal{J}]^{-}}{[\nabla \mathcal{J}]^{+}}\right)^{\eta}
\end{equation}
where $\odot$ represents Hadamard product (elementwise product) and $(\centerdot)^{\eta}$ denotes the elementwise power and $\eta (0<\eta \leq 1)$ is a learning rate. 
It can be easily seen that the multiplicative update \eqref{equ: J = X-U1W1V1} preserves the nonnegativity of the parameter $\Theta$, while $\nabla \mathcal{J} = 0$ when the convergence is achieved.
With these gradient calculations, the rule \eqref{equ: Theta <- Theta} with $\eta = 1$ yields the multiplicative updates on Stiefel manifolds to achieve orthogonal non-negative matrix tri-factorization by
\begin{align}
    U_{1} &\leftarrow U_{1} \odot \frac{XV_{1}W_{1}^{\top}}{U_{1}W_{1}V_{1}^{\top}X^{\top}U_{1}} \label{equ: update U1}\\
    V_{1} &\leftarrow V_{1}\odot\frac{X^{\top}U_{1}W_{1}}{V_{1}W_{1}^{\top}U_{1}^{\top}XV_{1}}\label{equ: update V1}\\
    W_{1} &\leftarrow W_{1}\odot\frac{U_{1}^{\top}XV_{1}}{U_{1}^{\top}U_{1}W_{1}V_{1}^{\top}V_{1}}\label{equ: update W1}
\end{align}
In SAR imaging, the extracted nonlinear ASC feature $P_{ASC}^{i} \in \mathbb{R}^{r \times r}\quad (i = 1,2,\cdots,k)$ can be considered a linear accumulation after co-clustering. 
Once the low-rank principal components $W_{i}$ are extracted from the SAR imaging, we perform non-negative matrix tri-factorization on $W_{i}\in \mathbb{R}^{r \times r}$ with constraints,
\begin{equation}
    W_{i}\approx U_{i+1}W_{i+1}V_{i+1}^{\top}, \quad W_{i}-W_{i+1}=P_{ASC}^{i} 
\end{equation}
where the condition $W_{i}-W_{i+1}=P_{ASC}^{i}$ implies that the ASC feature in the image is a superposition of layers and $U_{i+1}, V_{i+1}\in \mathbb{R}^{r \times r}$.
Therefore, the problem of extracting nonlinear ASC features in SAR images can be transformed into a constrained non-negative matrix factorization problem,
\begin{equation}\label{equ: non-negative matrix factorization with constraints problem}
\begin{aligned}
& \underset{U_{i+1}\geq 0,V_{i+1}\geq 0}{\text{minimize}}
& & \mathcal{G}(U_{i+1},V_{i+1}) = \frac{1}{2}\|W_{i}-U_{i+1}W_{i+1}V_{i+1}^{\top}\|_{F}^{2}  \\
& \text{subject to}
& & W_{i}-W_{i+1}=P_{ASC}^{i}.
\end{aligned}
\end{equation}
Note that the process of iteratively finding the next layer $W_{i+1}$ is a clustering process. 
According to the theory of orthogonal non-negative matrix factorization \cite{ding2005equivalence}, as long as $V_{i+1}$ is an orthogonal matrix, solving \eqref{equ: non-negative matrix factorization with constraints problem} is equivalent to a k-means clustering problem. 
At this point, the constrained optimization \eqref{equ: non-negative matrix factorization with constraints problem} is transformed into,
\begin{equation}\label{equ: orthogonal non-negative matrix factorization with constraints problem}
\begin{aligned}
& \underset{U_{i+1}\geq 0,V_{i+1}\geq 0}{\text{minimize}}
& & \mathcal{G}(U_{i+1},V_{i+1}) = \frac{1}{2}\|W_{i}-U_{i+1}W_{i+1}V_{i+1}^{\top}\|_{F}^{2}  \\
& \text{subject to}
& & W_{i}-W_{i+1}=P_{ASC}^{i}, \quad V_{i+1}^{\top}V_{i+1}=I.
\end{aligned}
\end{equation}
By substituting $W_{i}-W_{i+1}=P_{ASC}^{i}$ from the constraint into the optimization problem, \eqref{equ: orthogonal non-negative matrix factorization with constraints problem} can be transformed into an orthogonal non-negative matrix factorization problem,
\begin{equation}\label{equ: orthogonal non-negative matrix factorization problem}
\begin{aligned}
& \underset{U_{i+1},V_{i+1}}{\text{minimize}}
& & \mathcal{G}(U_{i+1},V_{i+1}) = \frac{1}{2}\|W_{i}-U_{i+1}(W_{i}-P_{ASC}^{i})V_{i+1}^{\top}\|_{F}^{2}  \\
& \text{subject to}
& &  U_{i+1}\geq 0,\quad V_{i+1}\geq 0, \quad V_{i+1}^{\top}V_{i+1}=I.
\end{aligned}
\end{equation}
To solve this optimization problem \eqref{equ: orthogonal non-negative matrix factorization problem}, we can adopt the algorithm update strategy from problem \eqref{equ: J = X-U1W1V1}.
First, we consider $U_{i+1}$, whose gradient in $\mathcal{G}$ is given by
\begin{equation}\label{equ: nabla Ui G}
    \begin{aligned}
        \nabla_{U_{i+1}} \mathcal{G} & = - W_{i}V_{i+1}(W_{i}-P_{ASC}^{i})^{\top}  \\
        & + U_{i+1}(W_{i}-P_{ASC}^{i})V_{i+1}^{\top}V_{i+1}(W_{i}-P_{ASC}^{i})^{\top}\\
        & = - W_{i}V_{i+1}(W_{i}-P_{ASC}^{i})^{\top} \\
        & +U_{i+1}(W_{i}-P_{ASC}^{i})(W_{i}-P_{ASC}^{i})^{\top}.
    \end{aligned}
\end{equation}
Note that $V_{i+1}$ is non-negative and orthogonal.
Minimizing such matrices $V_{i+1}$ has been well studied \cite{smith1993geometric,edelman1998geometry}.
The orthogonality constraint on $V_{i+1}$ is a restriction on the Stiefel manifold \cite{stiefel1935richtungsfelder}.
The gradient on the Stiefel manifold can be calculated using
\begin{equation}\label{equ: nabla Vi G = nabla Vi G - Vi nabla Vi G Vi}
    \widetilde{\nabla}_{V_{i+1}} \mathcal{G} = \nabla_{V_{i+1}} \mathcal{G} - V_{i+1} (\nabla_{V_{i+1}} \mathcal{G})^{\top}V_{i+1} .
\end{equation}
The gradient $\nabla_{V_{i+1}} \mathcal{G}$ can be computed as
\begin{equation}\label{equ: nabla Vi G = -WU(W-P) +V(W-P)UU(W-P)}
    \begin{aligned}
        \nabla_{V_{i+1}} \mathcal{G} & = -W_{i}^{\top}U_{i+1}(W_{i}-P_{ASC}^{i}) \\
        &+V_{i+1}(W_{i}-P_{ASC}^{i})^{\top}U_{i+1}^{\top}U_{i+1}(W_{i}-P_{ASC}^{i}).
    \end{aligned}
\end{equation}
Substituting \eqref{equ: nabla Vi G = -WU(W-P) +V(W-P)UU(W-P)} into \eqref{equ: nabla Vi G = nabla Vi G - Vi nabla Vi G Vi} yields the gradient on the Stiefel manifold,
\begin{equation}\label{equ: nabla V G in Stiefel manifold}
    \begin{aligned}
        \widetilde{\nabla}_{V_{i+1}} \mathcal{G} & = - W_{i}^{\top}U_{i+1}(W_{i}-P_{ASC}^{i}) \\
        & + V_{i+1}(W_{i}-P_{ASC}^{i})^{\top}U_{i+1}^{\top}W_{i}V_{i+1}
    \end{aligned}
\end{equation}
The optimization problem \eqref{equ: orthogonal non-negative matrix factorization problem} can be solved through the following iterative updates,
\begin{equation}\label{equ: Wi+1 Hi+1 update in ONMF}
    \begin{aligned}
        V_{i+1} &\leftarrow V_{i+1}\odot\frac{W_{i}^{\top}U_{i+1}(W_{i}-P_{ASC}^{i})}{V_{i+1}(W_{i}-P_{ASC}^{i})^{\top}U_{i+1}^{\top}W_{i}V_{i+1}}\\
        U_{i+1} &\leftarrow U_{i+1}\odot \frac{W_{i}V_{i+1}(W_{i}-P_{ASC}^{i})^{\top}}{U_{i+1}(W_{i}-P_{ASC}^{i})(W_{i}-P_{ASC}^{i})^{\top}}\\
    \end{aligned}
\end{equation}
Based on the previous description, we can utilize multi-layer orthogonal non-negative matrix factorization on the data matrix $X$ to incorporate the extracted nonlinear ASC features into different layers,
\begin{align}
    X \approx U_{1}W_{1}V_{1},&  \label{equ: X U1W1V1} \\
    W_{1}\approx U_{2}W_{2}V_{2}^{\top},& \quad W_{1}-W_{2}=P_{ASC}^{1} \label{equ: W1=U2W2V2}\\
    W_{2}\approx U_{3}W_{3}V_{3}^{\top},& \quad W_{2}-W_{3}=P_{ASC}^{2} \label{equ: W2=U3W3V3}\\
    \cdots &\nonumber\\
    W_{k}\approx U_{k+1}W_{k+1}V_{k+1}^{\top},& \quad W_{k+1}-W_{k}=P_{ASC}^{k} \label{equ: Wk=Uk+1Wk+1Vk+1}
\end{align}


==> material/related_work_NMF.tex <==

\subsection{Nonnegative Matrix Factorization}\label{sec: Nonnegative Matrix Factorization}

Non-negative Matrix Factorization (NMF) is a dimensionality reduction technique that approximates a non-negative matrix $X$ as the product of two non-negative matrices $W$ and $H$.
Specifically, given a non-negative matrix $X\in \mathbb{R}^{m \times n}$ and a desired rank $r$, NMF seeks to find $W\in \mathbb{R}^{m \times r}$ and $H \in \mathbb{R}^{r \times n}$ such that,
\begin{equation}\label{equ: X approx WH}
    X \approx WH.
\end{equation}
To determine the matrices $W$ and $H$ in \eqref{equ: X approx WH}, we consider minimizing the Frobenius norm of the squared Euclidean distance as a discrepancy measure between the data $X$ and the model $WH$. 
The optimization problem can be formulated as follows,
\begin{equation}\label{equ: NMF problem}
    \mathcal{J}_{NMF}(W,H)=\frac{1}{2}\|X-WH\|_{F}^{2},\text{s.t. }W\geq 0, H\geq 0,
\end{equation}
where $\|\centerdot \|_{F}$ is the Frobenius norm.
The solution for the NMF problem has been widely studied in the past few years \cite{lee2000algorithms,li2006relationships,ding2005equivalence,choi2008algorithms}.
Lee and Seung's \cite{lee2000algorithms} multiplicative update rule has been a popular method due to the simplicity of implementation. 
When applied to \eqref{equ: NMF problem}, the multiplicative update becomes
\begin{align}
    H &\leftarrow H\odot \frac{W^{\top}X}{W^{\top}WH}, \label{equ: H update in NMF}\\
    W &\leftarrow W\odot\frac{XH^{\top}}{WHH^{\top}}.\label{equ: W update in NMF}
\end{align}

==> not_used/name.tex <==
\section{Related Works}
\label{2}

\subsection{SAR ATR with Limited Data} 

\subsection{Causal Inference}
Causal inference is a fundamental problem in machine learning and has been the subject of extensive research in recent years. Many existing works in causal inference can be broadly categorized into two categories: causal discovery and causal effect estimation.

Causal discovery aims to infer the causal structure of a system from observational data. A popular approach in causal discovery is to use graphical models, such as Bayesian networks [14] and causal Bayesian networks [15], to represent the causal relationships between variables. Other methods include constraint-based algorithms [16] and information-theoretic methods [17].

Causal effect estimation, on the other hand, aims to estimate the causal effect of a treatment on an outcome. This is often done using randomized controlled trials (RCTs), where the treatment is randomly assigned to the subjects. However, in many cases, RCTs are not feasible or ethical, and we need to rely on observational data. In this case, we can use methods such as propensity score matching [18] and inverse probability weighting [19] to estimate the causal effect.

Recently, there has been a growing interest in developing methods for causal inference in the presence of confounders, where the treatment and outcome are affected by common causes. These methods aim to control for confounding variables by either adjusting for them in the analysis or by using experimental designs that minimize their impact [20]. One popular approach is the use of instrumental variables, which are variables that affect the treatment but not the outcome, to estimate the causal effect [21].

In addition to these methods, there has been increasing interest in the use of deep learning for causal inference. Deep learning models can be used to estimate causal effects from observational data by learning the functional form of the causal relationship between variables [22]. Some recent works have also explored the use of deep learning for causal discovery [23,24]. However, the use of deep learning for causal inference is still in its early stages, and more research is needed to fully explore its potential.
